A Construction for Variable Dimension Strong Non-Overlapping Matrices

We propose a method for the construction of sets of variable dimension strong non-overlapping matrices basing on any strong non-overlapping set of strings.

==> eptcsdata.tex <==
\providecommand{\firstpage}{25}
\providecommand{\publicationstatus}{Zs. Gazdag, Sz. Iv\'an, G. Kov\'asznai (Eds.): 16th International\\Conference on Automata and Formal Languages (AFL 2023)\\
EPTCS 386, 2023, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.386.4}{10.4204/EPTCS.386.4}}
\pdfoutput=1

